The Mixture Graph-A Data Structure for Compressing, Rendering, and Querying Segmentation Histograms

In this paper, we present a novel data structure, called the Mixture Graph. This data structure allows us to compress, render, and query segmentation histograms. Such histograms arise when building a mipmap of a volume containing segmentation IDs. Each voxel in the histogram mipmap contains a convex combination (mixture) of segmentation IDs. Each mixture represents the distribution of IDs in the respective voxel's children. Our method factorizes these mixtures into a series of linear interpolations between exactly two segmentation IDs. The result is represented as a directed acyclic graph (DAG) whose nodes are topologically ordered. Pruning replicate nodes in the tree followed by compression allows us to store the resulting data structure efficiently. During rendering, transfer functions are propagated from sources (leafs) through the DAG to allow for efficient, pre-filtered rendering at interactive frame rates. Assembly of histogram contributions across the footprint of a given volume allows us to efficiently query partial histograms, achieving up to 178$\times$ speed-up over na$\mathrm{\"{i}}$ve parallelized range queries. Additionally, we apply the Mixture Graph to compute correctly pre-filtered volume lighting and to interactively explore segments based on shape, geometry, and orientation using multi-dimensional transfer functions.

==> The Mixture Graph Preprint/FAfigure.tex <==
\begin{figure}[tb]
\centering

\begin{tikzpicture}[scale=0.65, every node/.style={scale=0.65}]

	%% SUBFIGURE TO THE RIGHT -- TESSELATION
	\begin{scope}[shift={(5.2cm,0.0cm)}]
		\draw[step=0.4cm,gray,very thin] (0.6,-0.2) grid(4.4,5.4);

		\filldraw[fill=clr9] (1.2,-0.4) rectangle (1.6,0);
		\filldraw[fill=clr7] (1.6,-0.4) rectangle (3.2,0);
		\filldraw[fill=clr8] (3.2,-0.4) rectangle (4,0);
		\begin{scope}[shift={(0.2cm,0)}]% X-labels
			\foreach \x in {2,3,4,5,6,7,8,9,10} \draw (\x*0.4 cm,0) node[anchor=north] {$\x$};
		\end{scope}

		\filldraw[fill=clr9] (0.4,1.2) rectangle (0.8,1.6);
		\filldraw[fill=clr7] (0.4,1.6) rectangle (0.8,3.2);
		\filldraw[fill=clr7] (0.4,3.2) rectangle (0.8,4.8);
		\begin{scope}[shift={(0.8,0.2cm)}]% Y-labels
			\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12} \draw(0.08,\y*0.4 cm) node[anchor=east] {$\y$};
		\end{scope}

		\draw[black,thin] (0.6,0) -- (4.6,0);
		\draw[black,thin] (0.8,-0.2) -- (0.8,5.4);

		\begin{scope}[shift={(1.2,0.4)}]% 1x1 squares
			\foreach \x in {0,1,2,3,4,5,6} \filldraw[fill=clr9] (\x*0.4,0.8) rectangle(\x*0.4 + 0.4,1.2);
		\end{scope}

		\begin{scope}[shift={(1.2,1.6)}]% 1x1 squares
			\foreach \y in {0,1,2,3,4,5,6,7} \filldraw[fill=clr9] (0,\y*0.4) rectangle (0.4,\y*0.4 + 0.4);
		\end{scope}
	
		\begin{scope}[shift={(1.6,1.6)}]% 4x4 squares
			\foreach \y in {0,1} {
				\filldraw[fill=clr7] (0,\y*1.6) rectangle(1.6,\y*1.6+1.6);
				\draw[step=0.4cm,clr6,very thin] (0.02,\y*1.6+0.02) grid (1.58,\y*1.6+1.58);
			}
		\end{scope}

		\begin{scope}[shift={(3.2,1.6)}]
			\foreach \y in {0,1,2,3} {
				\filldraw[fill=clr8] (0,\y*0.8) rectangle(0.8,\y*0.8+0.8);
				\draw[step=0.4cm,clr6,very thin] (0.02,\y*0.8+0.02) grid (0.78,\y*0.8+0.78);
			}
		\end{scope}
	\end{scope} %% END TESSELATION SUBFIGURE


%% grid
\draw[step=0.4cm,gray,very thin] (-0.2,-0.2) grid(5,5.4);

%% LEGEND X-AXIS
%% gray 1x1 boxes, 2x1 boxes, 4x1 boxes
\foreach \x in {0,1,2,4,5,6,7,8,9,10,11} \filldraw[fill=clr6] (\x*0.4,-1.7) rectangle (\x*0.4+0.4,-1.4);
\foreach \x in {0,1,2,3,5} \filldraw[fill=clr6] (\x*0.8,-1.3) rectangle (\x*0.8+0.8,-1);
\foreach \x in {0,2} \filldraw[fill=clr6] (\x*1.6,-0.9) rectangle (\x*1.6+1.6,-0.6);
%% blue boxes
\filldraw[fill=clr9] (1.2,-1.7) rectangle (1.6,-1.4);
\filldraw[fill=clr8] (3.2,-1.3) rectangle (4,-1);
\filldraw[fill=clr7] (1.6,-0.9) rectangle (3.2,-0.6);
%% labels of 1x1, 2x2, 4x4 legends on x-axis
\draw (-0.1,-1.55) node[anchor=east] {$0$};
\draw (-0.1,-1.15) node[anchor=east] {$1$};
\draw (-0.1,-0.75) node[anchor=east] {$2$};
%% boxes over numbers
\filldraw[fill=clr9] (1.2,-0.4) rectangle (1.6,0);
\filldraw[fill=clr7] (1.6,-0.4) rectangle (3.2,0);
\filldraw[fill=clr8] (3.2,-0.4) rectangle (4,0);
\begin{scope}[shift={(0.2cm,0)}]% X-labels
	\foreach \x in {0,1,2,3,4,5,6,7,8,9,10,11} \draw (\x*0.4 cm,0) node[anchor=north] {$\x$};
\end{scope}
\draw[decorate,decoration={brace,amplitude=4pt},xshift=0,yshift=0] (-0.4,-1.7) -- (-0.4,-0.6) node [black,midway,xshift=-0.4cm] {$l_x$};

\draw[black,thin] (-0.2,0) -- (5,0);
\draw[black,thin] (0,-0.2) -- (0,5.4);

\filldraw[fill=clr6] (-0.9,0) rectangle (-0.6,1.6);

\foreach \y in {1,2} \filldraw[fill=clr7] (-0.9,\y*1.6) rectangle (-0.6,\y*1.6+1.6);
\draw (-0.75,0) node[anchor=north] {$2$};
\foreach \y in {0,1,2,3,4,5} \filldraw[fill=clr6] (-1.3,\y*0.8) rectangle (-1,\y*0.8+0.8);
\draw (-1.15,0) node[anchor=north] {$1$};
\foreach \y in {0,1,2,4,5,6,7,8,9,10,11,12} \filldraw[fill=clr6] (-1.7,\y*0.4) rectangle (-1.4,\y*0.4+0.4);
\draw (-1.55,0) node[anchor=north] {$0$};
\filldraw[fill=clr9] (-1.7,1.2) rectangle (-1.4,1.6);
\draw[decorate,decoration={brace,amplitude=4pt,mirror},xshift=0,yshift=0] (-1.7,-0.35) -- (-0.6,-0.35) node [black,midway,yshift=-0.4cm] {$l_y$};

\filldraw[fill=clr6] (-0.9,4.8) rectangle (-0.6,5.42);
\filldraw[fill=clr6] (-1.3,4.8) rectangle (-1,5.42);
\fill[fill=white] (-1.72,5.35) rectangle (-0.58,5.45);

\filldraw[fill=clr9] (-0.4,1.2) rectangle (0,1.6);
\filldraw[fill=clr7] (-0.4,1.6) rectangle (0,3.2);
\filldraw[fill=clr7] (-0.4,3.2) rectangle (0,4.8);
\begin{scope}[shift={(0,0.2cm)}]% Y-labels
	\foreach \y in {0,1,2,3,4,5,6,7,8,9,10,11,12} \draw(0.08,\y*0.4 cm) node[anchor=east] {$\y$};
\end{scope}

%% TENSOR PRODUCT
\begin{scope}[shift={(1.2,1.2)}]
	\filldraw[fill=clr6] (0,0) rectangle (0.4,0.4);
	\filldraw[fill=clr6] (0.4,0) rectangle (2.0,0.4);
	\filldraw[fill=clr6] (2.0,0) rectangle (2.8,0.4);
	
	\filldraw[fill=clr6] (0,0.4) rectangle (0.4,2.0);
	\filldraw[fill=clr6] (0,2.0) rectangle (0.4,3.6);
	\filldraw[fill=clr6] (0.4,0.4) rectangle (2.0,2.0);
	\filldraw[fill=clr6] (0.4,2.0) rectangle (2.0,3.6);
	\filldraw[fill=clr6] (2.0,0.4) rectangle(2.8,2.0);
	\filldraw[fill=clr6] (2.0,2.0) rectangle(2.8,3.6);
\end{scope}

\end{tikzpicture}
\caption{\label{fig:footprint}Footprint assembly in 2D. \textbf{Left:} The 2D footprint formed by the tensor product of 1D footprints consists of rectangles. Alignments and extents of samples of the mimmap are shown next to each axis. \textbf{Right}: Rectangles in the 2d footprint are tesselated using squares matching the smaller side of each rectangle. Each square corresponds to one sample from the normalized histogram mipmap.}
\vspace{-4mm}
\end{figure}	


==> The Mixture Graph Preprint/dag.tex <==
\begin{figure}[t]
\centering
\resizebox{0.55\columnwidth}{!}{%
\begin{tikzpicture}
\node[shape=rectangle,draw=clr11,fill=clr7,minimum size=0.8cm] (1) at (0,0) {~~$\unit{1}$~~};
\node[shape=rectangle,draw=clr11,fill=clr7,minimum size=0.8cm] (2) at(2,0) {$\unit{2}$};
\node[shape=rectangle,draw=clr11,fill=clr7,minimum size=0.8cm] (3) at (4,0) {$\unit{3}$};
\node[shape=rectangle,draw=clr11,fill=clr7,minimum size=0.8cm] (4) at(6,0) {$\unit{4}$};

\node[shape=circle,draw=black,fill=clr6,minimum size=0.8cm] (5) at (1,1.5) {$\vc{\lambda}_5$};
\node[shape=circle,draw=black,fill=clr6,minimum size=0.8cm] (6) at (2,3) {$\vc{\lambda}_6$};
\node[shape=rounded rectangle,draw=clr1,fill=clr5,minimum size = 0.8cm] (7) at (3,4.5) {$\vc{m}\equiv\vc{\lambda}_7$};

\node[shape=circle,draw=black,fill=clr6,minimum size=0.8cm] (8) at (5,-1.5) {$\vc{\lambda}_8$};
\node[shape=rounded rectangle,draw=clr1,fill=clr5,minimum size = 0.8cm] (9) at (3,-2.4) {$\vc{m^\prime}\equiv\vc{\lambda}_9$};

\path[->, thick] (1) edge node[left] {\raisebox{12pt}{$\mathbf{\dfrac{1}{3}~}$}} (5);
\path[->, thick] (2) edge node[right] {\raisebox{12pt}{$\mathbf{~\dfrac{2}{3}}$}} (5);
\path[->, thick] (3) edge node[right] {\raisebox{12pt}{$\mathbf{~\dfrac{1}{2}}$}} (6);
\path[->, thick] (4) edge node[right] {\raisebox{12pt}{$\mathbf{~\dfrac{2}{5}}$}} (7);
\path[->, thick] (5) edge node[left] {\raisebox{12pt}{$\mathbf{\dfrac{1}{2}}~$}} (6);
\path[->, thick] (6) edge node[left]  {\raisebox{12pt}{$\mathbf{\dfrac{3}{5}}~$}} (7);
\path[->, thick] (3) edge node[left] {\raisebox{-18pt}{$\mathbf{\dfrac{1}{4}}~$}} (8);
\path[->, thick] (4) edge node[right] {\raisebox{-18pt}{$~\mathbf{\dfrac{3}{4}}$}} (8);
\path[->, thick] (8) edge[bend left] node[right] {\raisebox{-24pt}{$~\mathbf{\dfrac{2}{5}}$}} (9);
\path[->, thick] (5) edge[bend right] node[left] {\raisebox{-24pt}{$~\mathbf{\dfrac{3}{5}}$}} (9);
\end{tikzpicture}
}
\vspace{-2mm}
\caption{\label{fig:DAG}Example directed acyclic graph (DAG) corresponding to the factorization of $\vc{m}=\left(\;0.1,0.2,0.3,0.4,\ldots\;\right)$ and $\vc{m^\prime}=\left(\;0.2,0.4,0.1,0.3,\ldots\;\right)$. Mixture $\vc{\lambda}_5$ can be re-used, since the ratio between the first two components is the same ($0.1:0.2\;\equiv\;0.2:0.4$).}
\vspace{-4mm}
\end{figure}


==> The Mixture Graph Preprint/dagtopo.tex <==
\begin{figure}[b]
\vspace{-2mm}
\centering
\resizebox{0.85\columnwidth}{!}{%
\begin{tikzpicture}
\node[shape=rectangle,draw=clr11,fill=clr7,minimum size=0.8cm] (1) at (0,0) {$0$};
\node[shape=rectangle,draw=clr11,fill=clr7,minimum size=0.8cm] (2) at (2,0) {$0$};
\node[shape=rectangle,draw=clr11,fill=clr7,minimum size=0.8cm] (3) at (4,0) {$0$};
\node[shape=rectangle,draw=clr11,fill=clr7,minimum size=0.8cm] (4) at (6,0) {$0$};
\node[shape=rectangle,draw=clr11,fill=clr7,minimum size=0.8cm] (5) at (8,0) {$0$};

\node[shape=circle,draw=black,fill=clr4,minimum size=0.8cm] (6) at (1,1.5)  {$1$};
\node[shape=circle,draw=black,fill=clr7!50!clr8,minimum size=0.8cm] (7) at (7,1)  {$1$};

\node[shape=circle,draw=black,fill=clr8,minimum size=0.8cm] (9) at (6,2)  {$2$};

\node[shape=rounded rectangle,draw=black,fill=clr8!50!clr9,minimum size = 0.8cm] (10) at (4,3) {$3$};


\path[->, thick] (1) edge node[left] {} (6);
\path[->, thick] (2) edge node[right] {} (6);

\path[->, thick] (4) edge node[right] {} (7);
\path[->, thick] (5) edge node[right] {} (7);

\path[->, thick] (3) edge node[left] {} (9);
\path[->, thick] (7) edge node[left]  {} (9);

\path[->, thick] (6) edge node[left] {} (10);
\path[->, thick] (9) edge node[right] {} (10);

\end{tikzpicture}
}
\caption{\label{fig:dagtopo}Topological sorting of the DAG. Node numbers indicate the distance to the closest source. During parallel reconstruction smaller numbers have to be processed before larger numbers. The largest number corresponds sto the number of synchronization steps required. Here, the orange node has only successors with a value of 3. It can be processed together with nodes labelled '$1$' or with nodes labelled '$2$'.}
\end{figure}


==> The Mixture Graph Preprint/factorization.tex <==
\begin{figure}[t]
\centering
	\fbox{
		\begin{minipage}{0.75\columnwidth}
		\footnotesize
		\renewcommand{\arraystretch}{1.2}
		\centering
		\begin{tabular}{ll}
			Input:     & $\vc{m}=\left(\;0.1,0.2,0.3,0.4,\ldots\;\right)$\\
			Mixture List: & $\Lambda=\left[\;\unit{1},\unit{2},\unit{3},\unit{4}\;\right]$\vspace{0.5mm}\\
			\hline\\[-2.5ex]
%%
			Pick ${\color{clr1}\mathbf{1}},{\color{clr3}\mathbf{2}}$:  & $\vc{m}=\left(\;{\color{clr1}\mathbf{0.1}},{\color{clr3}\mathbf{0.2}},0.3,0.4,\ldots\;\right)$\\
			Insert new ${\color{clr10}\mathbf{\lambda}}$: &
			{\tabcolsep0pt
				\begin{tabular}{l}
					$\Lambda = \left[\;\unit{1},\unit{2},\unit{3},\unit{4},{\color{clr10}\mathbf{\vc{\lambda}_5}}\;\right]$,\\
					${\color{clr10}\mathbf{\vc{\lambda}_5}}=\frac{1}{3}\left(\;{\color{clr1}\mathbf{1}},{\color{clr3}\mathbf{2}},\ldots\;\right)$					
				\end{tabular}
			}\\
		Update: & $\vc{m}=\left(\;{\color{clr10}{\mathbf{0}}},{\color{clr10}{\mathbf{0}}},0.3,0.4,{\color{clr10}{\mathbf{0.3}}},\ldots\;\right)$\vspace{0.5mm}\\
		\hline\\[-2.5ex]
%%
			Pick ${\color{clr1}\mathbf{3}},{\color{clr3}\mathbf{5}}$: & $\vc{m}=\left(\;0,0,{\color{clr1}\mathbf{0.3}},0.4,{\color{clr3}\mathbf{0.3}},\ldots\;\right)$\\
			Insert new ${\color{clr10}\mathbf{\lambda}}$: &
			{\tabcolsep0pt
				\begin{tabular}{l}
					$\Lambda = \left[\;\unit{1},\unit{2},\unit{3},\unit{4},\vc{\lambda}_5,{\color{clr10}\mathbf{\vc{\lambda}_6}}\;\right]$,\\
			${\color{clr10}\mathbf{\vc{\lambda}_6}}=\frac{1}{2}\left(\;0,0,{\color{clr1}\mathbf{1}},0,{\color{clr3}\mathbf{1}},\ldots\;\right)$\\					
				\end{tabular}
			}\\
		Update: & $\vc{m} = \left(\;0,0,{\color{clr10}\mathbf{0}},0.4,{\color{clr10}\mathbf{0}},{\color{clr10}\mathbf{0.6}},\ldots\;\right)$\vspace{0.5mm}\\
		\hline\\[-2.5ex]
		
		Pick ${\color{clr1}\mathbf{4}},{\color{clr3}\mathbf{6}}$: & $\vc{m}=\left(\;0,0,0,{\color{clr1}\mathbf{0.4}},0,{\color{clr3}\mathbf{0.6}},\ldots\;\right)$\\
		Insert new ${\color{clr10}\mathbf{\lambda}}$: &
		{\tabcolsep0pt
			\begin{tabular}{l}
				$\Lambda = \left[\;\unit{1},\unit{2},\unit{3},\unit{4},\vc{\lambda}_5,\vc{\lambda}_6,{\color{clr10}\mathbf{\vc{\lambda}_7}}\;\right]$,\\
				${\color{clr10}\mathbf{\vc{\lambda}_7}} = \frac{1}{5}\left(\;0,0,0,{\color{clr1}\mathbf{2}},0,{\color{clr3}\mathbf{3}},\ldots\;\right)$\\
			\end{tabular}
		}\\
		Update: & $\vc{m}=\left(\;0,0,0,{\color{clr10}\mathbf{0}},0,{\color{clr10}\mathbf{0}},{\color{clr10}\mathbf{1}},\ldots\;\right)$\vspace{0.5mm}\\
	\hline\\[-2.5ex]
%%
			Result: & 
			{\tabcolsep0pt
				\begin{tabular}{l}
				$\vc{m} = \left(\;0,0,0,0,0,0,1\ldots\;\right)$\\
			  $\Lambda = \left[\;\unit{1},\unit{2},\unit{3},\unit{4},\vc{\lambda}_5,\vc{\lambda}_6,\vc{\lambda}_7\;\right]$.
				\end{tabular}
			}
		\end{tabular}
		\end{minipage}
	}
	\vspace{-1mm}
\caption{\label{fig:factorization}Factorization of a mixture $\vc{m}$, $\|\vc{m}\|_0=4$. In each step, two non-zero positions in $\vc{m}$ are selected, a new linear interpolation $\lambda$ is added to the mixture list $\Lambda$, and $\vc{m}$ is updated ($\ldots$ denote \hl{trailing} zeros).}
\vspace{-4mm}
\end{figure}

==> The Mixture Graph Preprint/trash.tex <==
%% TODO: USE THIS FOR HEINZL DATA AFTER
%% GROUND TRUTH IS DONE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%To reduce the processing time, we increased $\tau$ to 5 during the first stages of the factorization, thereby exempting mixtures with fewer components from the greedy search, but not the factorization steps. Once the score of the index pairs to be factored out reached a threshold $\phi_2<5000$, we decreased $\tau$ to 4 and then again at $\phi_2<2000$ to 3. \\


%% OLD TABLE 2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{table}
%\caption{\label{tab:results1}Mixture graph results for the Hippocampus dataset \cite{Cali16} depicted in Fig.~\ref{fig:teaser}, left. 
%We compare results for both the max-occurence (Eqn.~\eqref{eq:greedy1}) and the max-reduction (Eqn.~\eqref{eq:greedy2}) strategies. As can be seen, picking the factorization that minimizes the remaining search space using the max-reduction strategy results in a slightly better fidelity and a substantially reduced encoding time.}
%\centering
%\begin{tabular}{l|c|c}
%~ 								& \multicolumn{2}{|c}{\textbf{Input}}\\
%\hline
%Resolution 				& \multicolumn{2}{|c}{$1178\times1125\times789$}\\
%Mip Levels 				& \multicolumn{2}{|c}{12}\\
%Segments  				& \multicolumn{2}{|c}{256}\\
%Background 				& \multicolumn{2}{|c}{47.74~\%}\\
%\multicolumn{3}{c}{}\\
%~ 								& \multicolumn{2}{|c}{\textbf{Histogram Mipmap}}\\
%\hline
%non-zeros/voxel		& \multicolumn{2}{|c}{1.007}\\
%raw size 					& \multicolumn{2}{|c}{13.43~GB}\\
%input node pairs 	& \multicolumn{2}{|c}{4'915'899}\\
%\multicolumn{3}{c}{}\\
%~ 								& \multicolumn{2}{|c}{\textbf{Mixture Graph}}\\
%~ 								& max-occurrence 	& max-reduction\\
%\hline
%nodes 						& $1'029'933$ 		& $1'029'188$ \\
%size 							& 1.36~GB 				& 1.36~GB\\
%bits/voxel				& 11.17           & 11.17\\
%quant. bins 			& 512 						& 512\\
%max error 				& 0.005240 				& 0.004878\\
%longest path 			& 11 							& 11\\
%encoding time 		& 21.8~min				& 8.32~min\\
%\end{tabular}
%\end{table}
%
%\begin{table}
%\caption{\label{tab:results2}Mixture graph results for a section of the Neocortex dataset \cite{Kasthuri15} depicted in Fig.~\ref{fig:teaser}, right. Similar to Table~\ref{tab:results1}, we compare results for both greedy strategies and note that the max-reduction strategy again results in better peformance. In parentheses, we list results for gradually lowering the cutoff threshold $\tau$.}
%\centering
%\begin{tabular}{l|c|c}
%~ 								& \multicolumn{2}{|c}{\textbf{Input}}\\
%\hline
%Resolution				& \multicolumn{2}{|c}{$2048\times 2048\times 300$}\\
%Mip Levels				& \multicolumn{2}{|c}{12}\\
%Segments					& \multicolumn{2}{|c}{1182}\\
%Background				& \multicolumn{2}{|c}{20.70~\%}\\
%\multicolumn{3}{c}{}\\
%~ 								& \multicolumn{2}{|c}{\textbf{Histogram Mipmap}}\\
%\hline
%non-zeros/voxel		& \multicolumn{2}{|c}{1.025}\\
%raw size					& \multicolumn{2}{|c}{16.34~GB}\\
%input node pairs	& \multicolumn{2}{|c}{$23'551'565$}\\
%\multicolumn{3}{c}{}\\
%~									& \multicolumn{2}{|c}{\textbf{Mixture Graph}}\\
%~									& max-occurrence 	& max-reduction\\
%\hline
%nodes							&	$5'305'970$			&	$5'300'258$ 	\\
%size							&	2.18~GB   			&	2.18~GB	  		\\
%bits/voxel				&	14.88 					&	14.88 				\\
%quant. bins				& 512							& 512						\\
%max error					&	0.005456				&	0.005225		 \\
%longest path			&	22							&	22						\\
%encoding time			&	7.86~h					&	2.89~h		\\
%\end{tabular}
%\end{table}

==> The Mixture Graph Preprint/tree.tex <==
\begin{figure}[b]
\centering
\resizebox{0.55\columnwidth}{!}{%
\begin{tikzpicture}
\node[shape=rectangle,draw=clr11,fill=clr7,minimum size=0.8cm] (1) at (0,0) {~~$\unit{1}$~~};
\node[shape=rectangle,draw=clr11,fill=clr7,minimum size=0.8cm] (2) at(2,0) {$\unit{2}$};
\node[shape=rectangle,draw=clr11,fill=clr7,minimum size=0.8cm] (3) at (4,0) {$\unit{3}$};
\node[shape=rectangle,draw=clr11,fill=clr7,minimum size=0.8cm] (4) at(6,0) {$\unit{4}$};

\node[shape=circle,draw=black,fill=clr6,minimum size=0.8cm] (5) at (1,1.5) {$\vc{\lambda}_5$};
\node[shape=circle,draw=black,fill=clr6,minimum size=0.8cm] (6) at (2,3) {$\vc{\lambda}_6$};
\node[shape=rounded rectangle,draw=clr1,fill=clr5,minimum size = 0.8cm] (7) at (3,4.5) {$\vc{m}\equiv\vc{\lambda}_7$};

\path[->, thick] (1) edge node[left] {\raisebox{12pt}{$\mathbf{\dfrac{1}{3}~}$}} (5);
\path[->, thick] (2) edge node[right] {\raisebox{12pt}{$\mathbf{~\dfrac{2}{3}}$}} (5);
\path[->, thick] (3) edge node[right] {\raisebox{12pt}{$\mathbf{~\dfrac{1}{2}}$}} (6);
\path[->, thick] (4) edge node[right] {\raisebox{12pt}{$\mathbf{~\dfrac{2}{5}}$}} (7);
\path[->, thick] (5) edge node[left] {\raisebox{12pt}{$\mathbf{\dfrac{1}{2}}~$}} (6);
\path[->, thick] (6) edge node[left]  {\raisebox{12pt}{$\mathbf{\dfrac{3}{5}}~$}} (7);
\end{tikzpicture}
}
\vspace{-1mm}
\caption{\label{fig:tree}Factorization tree of the example in Fig.~\ref{fig:factorization}. Leaf nodes (boxes) store unit vectors representing the input segment IDs, internal nodes (circles) perform linear interpolations between two children, and the root (rounded rectangle) corresponds to the original mixture $\vc{m}$.}
\end{figure}

==> trash.tex <==
%% TODO: USE THIS FOR HEINZL DATA AFTER
%% GROUND TRUTH IS DONE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%To reduce the processing time, we increased $\tau$ to 5 during the first stages of the factorization, thereby exempting mixtures with fewer components from the greedy search, but not the factorization steps. Once the score of the index pairs to be factored out reached a threshold $\phi_2<5000$, we decreased $\tau$ to 4 and then again at $\phi_2<2000$ to 3. \\


%% OLD TABLE 2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\begin{table}
%\caption{\label{tab:results1}Mixture graph results for the Hippocampus dataset \cite{Cali16} depicted in Fig.~\ref{fig:teaser}, left. 
%We compare results for both the max-occurence (Eqn.~\eqref{eq:greedy1}) and the max-reduction (Eqn.~\eqref{eq:greedy2}) strategies. As can be seen, picking the factorization that minimizes the remaining search space using the max-reduction strategy results in a slightly better fidelity and a substantially reduced encoding time.}
%\centering
%\begin{tabular}{l|c|c}
%~ 								& \multicolumn{2}{|c}{\textbf{Input}}\\
%\hline
%Resolution 				& \multicolumn{2}{|c}{$1178\times1125\times789$}\\
%Mip Levels 				& \multicolumn{2}{|c}{12}\\
%Segments  				& \multicolumn{2}{|c}{256}\\
%Background 				& \multicolumn{2}{|c}{47.74~\%}\\
%\multicolumn{3}{c}{}\\
%~ 								& \multicolumn{2}{|c}{\textbf{Histogram Mipmap}}\\
%\hline
%non-zeros/voxel		& \multicolumn{2}{|c}{1.007}\\
%raw size 					& \multicolumn{2}{|c}{13.43~GB}\\
%input node pairs 	& \multicolumn{2}{|c}{4'915'899}\\
%\multicolumn{3}{c}{}\\
%~ 								& \multicolumn{2}{|c}{\textbf{Mixture Graph}}\\
%~ 								& max-occurrence 	& max-reduction\\
%\hline
%nodes 						& $1'029'933$ 		& $1'029'188$ \\
%size 							& 1.36~GB 				& 1.36~GB\\
%bits/voxel				& 11.17           & 11.17\\
%quant. bins 			& 512 						& 512\\
%max error 				& 0.005240 				& 0.004878\\
%longest path 			& 11 							& 11\\
%encoding time 		& 21.8~min				& 8.32~min\\
%\end{tabular}
%\end{table}
%
%\begin{table}
%\caption{\label{tab:results2}Mixture graph results for a section of the Neocortex dataset \cite{Kasthuri15} depicted in Fig.~\ref{fig:teaser}, right. Similar to Table~\ref{tab:results1}, we compare results for both greedy strategies and note that the max-reduction strategy again results in better peformance. In parentheses, we list results for gradually lowering the cutoff threshold $\tau$.}
%\centering
%\begin{tabular}{l|c|c}
%~ 								& \multicolumn{2}{|c}{\textbf{Input}}\\
%\hline
%Resolution				& \multicolumn{2}{|c}{$2048\times 2048\times 300$}\\
%Mip Levels				& \multicolumn{2}{|c}{12}\\
%Segments					& \multicolumn{2}{|c}{1182}\\
%Background				& \multicolumn{2}{|c}{20.70~\%}\\
%\multicolumn{3}{c}{}\\
%~ 								& \multicolumn{2}{|c}{\textbf{Histogram Mipmap}}\\
%\hline
%non-zeros/voxel		& \multicolumn{2}{|c}{1.025}\\
%raw size					& \multicolumn{2}{|c}{16.34~GB}\\
%input node pairs	& \multicolumn{2}{|c}{$23'551'565$}\\
%\multicolumn{3}{c}{}\\
%~									& \multicolumn{2}{|c}{\textbf{Mixture Graph}}\\
%~									& max-occurrence 	& max-reduction\\
%\hline
%nodes							&	$5'305'970$			&	$5'300'258$ 	\\
%size							&	2.18~GB   			&	2.18~GB	  		\\
%bits/voxel				&	14.88 					&	14.88 				\\
%quant. bins				& 512							& 512						\\
%max error					&	0.005456				&	0.005225		 \\
%longest path			&	22							&	22						\\
%encoding time			&	7.86~h					&	2.89~h		\\
%\end{tabular}
%\end{table}
